Exploring the Potential of Flexible 8-bit Format: Design and Algorithm

Neural network quantization is widely used to reduce model inference complexity in real-world deployments. However, traditional integer quantization suffers from accuracy degradation when adapting to various dynamic ranges. Recent research has focused on a new 8-bit format, FP8, with hardware support for both training and inference of neural networks but lacks guidance for hardware design. In this paper, we analyze the benefits of using FP8 quantization and provide a comprehensive comparison of FP8 with INT quantization. Then we propose a flexible mixed-precision quantization framework that supports various number systems, enabling optimal selection of the most appropriate quantization format for different neural network architectures. Experimental results demonstrate that our proposed framework achieves competitive performance compared to full precision on various tasks, including image classification, object detection, segmentation, and natural language understanding. Our work furnishes critical insights into the tangible benefits and feasibility of employing FP8 quantization, paving the way for heightened neural network efficiency in tangible scenarios. Our code is available in the supplementary material.

==> LaTeX/tables/count.tex <==
\begin{table}[ht!]
    \begin{center}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l|llll}
        \toprule
        task & int8 & e5m2 & e4m3 & e3m4 & e2m5 \\
         \midrule
        cls. & 41 (not full) & 0 &1 &398 &2 \\
        det. & 22 & 0 & 0 & 713 & 4 \\
        seg. & 36 & 0 & 2 & 521 & 10 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \end{center}
    \caption{Allocation of all formats for tasks.}
    \label{tab:count}
\end{table}

==> LaTeX/tables/detailed_format_selection.tex <==
\begin{table*}[ht!]

    \begin{center}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lcccccccc}
        \toprule
        \multirow{2}{*}{\bf Task}  & \multirow{2}{*}{\bf Model} & \multicolumn{4}{c}{\bf INT8/E5M2/E4M3/E3M4/E2M5} & \multicolumn{3}{c}{\bf INT6/E3M2/E2M3} \\
        \cmidrule(l{2pt}r{2pt}){3-6}
        \cmidrule(l{2pt}r{2pt}){7-9}
        \multirow{2}{*}{} & \multirow{2}{*}{} & {Mixed FP8} & {Mixed FP8 ({\it r})} & {All Mixed} & {Limited Mix} & {Mixed FP6} & {All Mixed} & {Limited Mix} \\
        
        \midrule

        \multirow{6}{*}{Classification} & ResNet-18 & 0/0/0/75/1 & 22/12/1/41/0 & 1/0/0/75/0 & 0/0/0/75/1 & 0/75/1 & 1/75/0 & 1/75/0 \\
        \multirow{6}{*}{} & ResNet-50 & 0/0/0/156/2 & 64/34/0/60/0 & 2/0/0/156/0 & 0/0/0/156/2 & 0/156/2 & 2/156/0 & 2/156/0 \\
        \multirow{6}{*}{} & MobileNetv2 & 0/0/0/71/37 & 38/0/3/67/0 & 35/0/0/67/6 & 12/0/0/67/29 & 0/81/27 & 36/72/0 & 36/72/0 \\
        \multirow{6}{*}{} & RegNet3.2G & 0/0/0/288/1 & 53/46/9/155/0 & 2/0/0/287/0 & 2/0/0/287/0 & 0/220/69 & 98/191/0 & 0/288/1 \\
        \multirow{6}{*}{} & EfficientNet-b3 & 0/0/14/228/46 & 126/0/38/125/0 & 46/0/14/219/9 & 30/0/23/212/24 & 0/248/40 & 42/240/6 & 22/242/25 \\
        \multirow{6}{*}{} & ViT & 0/0/1/97/2 & 36/0/8/56/0 & 2/0/1/97/0 & 0/0/1/97/2 & 0/98/2 & 2/98/0 & 2/98/0 \\

        \midrule

        \multirow{4}{*}{Detection} & Retina-FPN & 0/0/0/162/10 & 53/37/1/81/0 & 10/0/0/162/0 & 0/0/0/162/10 & 0/162/10 & 10/162/0 & 10/162/0 \\
        \multirow{4}{*}{} & Faster-RCNN & 0/0/1/172/9 & 53/37/3/89/0 & 7/0/1/172/2 & 0/0/0/175/7 & 0/175/7 & 9/173/0 & 9/173/0 \\
        \multirow{4}{*}{} & YOLOX-m & 0/0/0/166/3 & 73/0/3/93/0 & 2/0/0/166/1 & 0/0/0/166/3 & 0/167/2 & 3/166/0 & 3/166/0 \\
        \multirow{4}{*}{} & YOLOX-l & 0/0/0/213/4 & 96/0/4/117/0 & 3/0/0/213/1 & 0/0/0/213/4 & 0/215/2 & 2/215/0 & 2/215/0 \\

        \midrule

        \multirow{4}{*}{Segmentation} & DeepLabv3-R50 & 0/0/0/209/5 & 77/46/2/73/0 & 1/0/0/209/4 & 1/0/0/210/3 & 0/210/4 & 4/210/0 & 4/210/0 \\
        \multirow{4}{*}{} & PSPNet-R50 & 0/0/1/200/9 & 77/44/2/71/0 & 5/0/1/200/4 & 8/0/0/200/2 & 0/202/8 & 8/202/0 & 8/202/0 \\
        \multirow{4}{*}{} & UNet-1024 & 0/0/0/55/5 & 23/15/2/20/0 & 4/0/0/55/1 & 2/0/0/56/2 & 0/56/4 & 3/56/1 & 3/56/1 \\
        \multirow{4}{*}{} & SegFormer-b0 & 0/0/1/61/23 & 38/4/3/40/0 & 26/0/1/57/1 & 14/0/1/59/11 & 0/64/21 & 24/61/0 & 24/61/0 \\
        
        
        % \multirow{6}{*}{Classification} & ResNet-18 & 70.28 & 69.73 & 70.17 & 69.77 & 70.13 & 70.17 \\
        % \multirow{6}{*}{(Top-1 Acc.)} & ResNet-50 & 76.76 & 76.17 & 76.70 &76.40 & 76.74 & 76.70 \\
        % \multirow{6}{*}{} & MobileNetv2 & 73.26 & 68.48 & 72.47 & 71.64 & 72.60 & 72.25 \\
        % \multirow{6}{*}{} & RegNet3.2G & 78.43 & 78.07 & 78.18 & 78.17 & 78.29 & 78.29 \\
        % \multirow{6}{*}{} & EfficientNet-b3 & 80.19 & 58.49 & 79.98 & 79.93 & 80.04 & 79.99 \\
        % \multirow{6}{*}{} & ViT & 83.15 & 82.67 & 83.08 & 83.06 & 83.17 & 83.08 \\
        % \midrule
        % \multirow{3}{*}{Detection} & Retina-FPN & 37.00 & 36.21 & 36.85 & 36.64 & 36.85 & 36.85 \\
        % \multirow{3}{*}{(mAP)} & Faster-RCNN & 38.27 & 37.53 & 38.21 & 37.57 & 38.16 & 38.21 \\
        % \multirow{3}{*}{} & YOLOX-m & 44.36 & 43.15 & 44.32 & 43.82 & 44.29 & 44.32 \\
        % \multirow{3}{*}{} & YOLOX-l & 47.35 & 45.96 & 47.27 & 46.81 & 47.35 & 47.27 \\
        % \midrule
        % \multirow{3}{*}{Segmentation} & DeepLabv3-R50 & 79.46 & 72.97 & 79.31 & 78.77 &79.32 & 79.31 \\
        % \multirow{3}{*}{(mIoU)} & PSPNet-R50 & 77.46 & 71.29 & 77.15 & 76.94 & 77.28 & 77.13 \\
        % \multirow{3}{*}{} & UNet-1024 & 67.40 & 65.28 & 67.33 & 66.93 & 67.31 & 67.28 \\
        % \multirow{3}{*}{} & SegFormer-b0 & 75.28 & 74.52 & 75.00 & 75.27 & 75.24 & 75.24 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \end{center}
    
    
    \caption{Detailed format selection for our experiments}
    \label{tab:detailed_format_selection}
\end{table*}

==> LaTeX/tables/detailed_fp_formats.tex <==
\begin{table*}[h!]
    \begin{center}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lllllll}
        \toprule
        \multirow{2}{*}{\bf Format} & \multicolumn{4}{c}{\bf 8-bit} & \multicolumn{2}{c}{\bf 6-bit} \\
        \cmidrule(l{2pt}r{2pt}){2-5}
        \cmidrule(l{2pt}r{2pt}){6-7}
         & {E5M2} & {E4M3} & {E3M4} & {E2M5} & {E3M2} & {E2M3} \\
         % & (IEEE 754) & (Nvidia) & (Ours) & (IEEE 754) & (Nvidia) & (Ours) \\
        \midrule
        Exponent bias & 15 & 7 & 3 & 1 & 3 & 1 \\
        Inf & N/A & N/A & N/A & N/A & N/A & N/A \\
        NaN & N/A & N/A & N/A & N/A & N/A & N/A \\
        Zeros & $S.00000.00$ & $S.0000.000$ & $S.000.0000$ & $S.00.00000$ & $S.000.00$ & $S.00.000$ \\
        Max normal & $ S.11110.11_2 $ & $ S.1110.111_2 $ & $ S.110.1111_2 $ & $ S.10.11111_2 $ & $ S.110.11_2 $ & $ S.10.111_2 $ \\
        Min normal & $ S.00001.00_2 $ & $ S.0001.000_2 $ & $ S.001.0000_2 $ & $ S.01.00000_2 $ & $ S.001.00_2 $ & $ S.01.000_2 $ \\
        Max subnormal & $ S.00000.11_2 $ & $ S.0000.111_2 $ & $ S.000.1111_2 $ & $ S.00.11111_2 $ & $ S.000.11_2 $ & $ S.00.111_2 $ \\
        Min subnormal & $ S.00000.01_2 $ & $ S.0000.001_2 $ & $ S.000.0001_2 $ & $ S.00.00001_2 $ & $ S.000.01_2 $ & $ S.00.001_2 $ \\
        
        % Exponent bias & 7 & 7 & 7 & 15 & 15 & 15\\
        % Inf & $S.1111.000_2$ & N/A & N/A & $S.11111.00_2$ & $S.11111.00_2$ & N/A \\
        % % NaN & \begin{tabular}[l]{@{}l@{}} $S.1111.\{001, \\010, 011, 100,\\101, 110, 111\}_2$ \end{tabular}
        % NaN & \begin{tabular}[l]{@{}l@{}} $S.1111.\{001, \\010, \ldots, 111\}_2$ \end{tabular} 
        % & $S.1111.111_2$ & N/A & \begin{tabular}[l]{@{}l@{}} $S.11111.\{01, 10, 11\}_2$ \end{tabular} & $S.11111.\{01, 10, 11\}_2$ & N/A \\
        % Zeros & $S.0000.000$ & $S.0000.000$ & $S.0000.000$ & $S.00000.00$ & $S.00000.00$ & $S.00000.00$ \\
        % Max normal & $ S.1110.111_2 $ & $ S.1111.110_2 $ & $ S.1110.111_2 $ & $ S.11110.11_2 $ & $ S.11110.11_2 $ & $ S.11110.11_2 $ \\
        % Min normal & $ S.0001.000_2 $ & $ S.0001.000_2 $ & $ S.0001.000_2 $ & $ S.00001.00_2 $ & $ S.00001.00_2 $ & $ S.00001.00_2 $ \\
        % Max subnormal & $ S.0000.111_2 $ & $ S.0000.111_2 $ & $ S.0000.111_2 $ & $ S.00000.11_2 $ & $ S.00000.11_2 $ & $ S.00000.11_2 $ \\
        % Min subnormal & $ S.0000.001_2 $ & $ S.0000.001_2 $ & $ S.0000.001_2 $ & $ S.00000.01_2 $ & $ S.00000.01_2 $ & $ S.00000.01_2 $ \\

        
        
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \end{center}
    \caption{The binary representation of different ours implementation for FP formats.}
    \label{tab:detailed_fp_formats}
\end{table*}

==> LaTeX/tables/extend.tex <==
\begin{table}[ht!]
    \begin{center}
    \begin{adjustbox}{max width=\textwidth}
    % \begin{tabular}{l|cc}
    %     \toprule
    %      & ours & ours-extend \\
    %      \midrule
    %     ResNet50 & 76.154 & 76.114 \\
    %     MobileNetv2 & 67.274 & 67.272 \\
    %     ViT & 82.872 & 82.870 \\
    %     \bottomrule
    % \end{tabular}

    \begin{tabular}{lccc}
        \toprule
         & {\bf ResNet-50} & {\bf MobileNetv2} & {\bf ViT} \\
         \midrule
         FP32 & 76.76 & 73.26 & 83.15 \\
         \midrule
         ours & 76.13 & 67.27 & 82.87 \\
         ours-extend & 76.11 & 67.27 & 82.87 \\
         \bottomrule
    \end{tabular}
    
    \end{adjustbox}
     \end{center}
    \caption{The impact of extending the upper limit for E4M3 format. }
    \label{tab:extend}
\end{table}

==> LaTeX/tables/llama.tex <==
\begin{table*}[ht!]
    \begin{center}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lccccccccc}
        \toprule
        \multirow{2}{*}{\bf Model} &\multirow{2}{*}{\bf Method} & \multicolumn{5}{c}{\bf MMLU} &\multirow{2}{*}{\bf GSM8K} &\multirow{2}{*}{\bf DROP} &\multirow{2}{*}{\bf HumanEval} \\
        % \cline{2-7}
        \cmidrule(l{2pt}r{2pt}){3-7}
        &&STEM & Humanities	& Social Sciences & Other & Avg. \\
        \midrule
        \multirow{7}{*}{LLaMA-7b} & FP16 & 31.48 & 39.2 & 37.75 & 36.94 & 35.81 & 10.08 & 27.83 & 12.8 \\
        \multirow{7}{*}{} & INT8 &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & NIA Format &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & Mixed FP8 &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & Mixed FP8(r) &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & All Mixed &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & Limited Mix &  &  &  &  &  &  &  &  \\
        \midrule
        \multirow{7}{*}{LLaMA-13b} & FP16 & 37.76 & 52.39 & 55.35 & 50.84 & 47.79 & 20.32 & 38.94 & 15.24 \\
        \multirow{7}{*}{} & INT8 &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & NIA Format &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & Mixed FP8 &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & Mixed FP8(r) &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & All Mixed &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & Limited Mix &  &  &  &  &  &  &  &  \\
        \midrule
        \multirow{7}{*}{LLaMA-30b} & FP16 & 46.92 & 64.75 & 67.36 & 60.77 & 58.44 & 42.38 & 48.76 & 20.73 \\
        \multirow{7}{*}{} & INT8 &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & NIA Format &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & Mixed FP8 &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & Mixed FP8(r) &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & All Mixed &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & Limited Mix &  &  &  &  &  &  &  &  \\
        \midrule
        \multirow{7}{*}{LLaMA-65b} & FP16 & 52.42 & 70.82 & 73.59 & 64.32 & 63.79 & 54.35 & 52.66 & 23.17  \\
        \multirow{7}{*}{} & INT8 &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & NIA Format &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & Mixed FP8 &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & Mixed FP8(r) &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & All Mixed &  &  &  &  &  &  &  &  \\
        \multirow{7}{*}{} & Limited Mix &  &  &  &  &  &  &  &  \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \end{center}
    \caption{Precision of various quantization formats on LLaMA models.}
    \label{tab:llama}
\end{table*}
